Single-particle detection of the N\'eel transition in LaCrO$_3$ microcrystals via widefield nitrogen-vacancy center magnetic imaging

We resolve the antiferromagnetic N\'eel transition in individual LaCrO$_3$ microcrystals using widefield nitrogen-vacancy (NV) magnetometry. Rare-earth orthochromites are canted antiferromagnets with rich, chemically tunable magnetic behavior, yet their magnetic ordering has been probed almost exclusively by ensemble techniques such as SQUID magnetometry and neutron diffraction. Here we image the stray magnetic fields of individual LaCrO$_3$ microcrystals produced via molten salt synthesis. Repeated thermal cycling through the N\'eel transition produces multiple micron-scale magnetic domains. Their locations recur from one cooldown to the next, but the sign of the staggered magnetization is set independently each time. We also observe temperature-independent signals in half of the particles, which we attribute to localized ferromagnetic impurities that are hidden in ensemble measurements. These results establish single-particle NV magnetometry as a probe of the N\'eel transition, domain structure, and impurity phases in canted antiferromagnetic microcrystals, opening a route to correlating magnetic ordering and domain formation with particle morphology and defect structure.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf';

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
